Joint Coordinate Regression and Association For Multi-Person Pose Estimation, A Pure Neural Network Approach

We introduce a novel one-stage end-to-end multi-person 2D pose estimation algorithm, known as Joint Coordinate Regression and Association (JCRA), that produces human pose joints and associations without requiring any post-processing. The proposed algorithm is fast, accurate, effective, and simple. The one-stage end-to-end network architecture significantly improves the inference speed of JCRA. Meanwhile, we devised a symmetric network structure for both the encoder and decoder, which ensures high accuracy in identifying keypoints. It follows an architecture that directly outputs part positions via a transformer network, resulting in a significant improvement in performance. Extensive experiments on the MS COCO and CrowdPose benchmarks demonstrate that JCRA outperforms state-of-the-art approaches in both accuracy and efficiency. Moreover, JCRA demonstrates 69.2 mAP and is 78\% faster at inference acceleration than previous state-of-the-art bottom-up algorithms. The code for this algorithm will be publicly available.

==> ablation.tex <==
\section{Ablation Studies}
To further understand the contribution of each component in the OmniDataComposer, we conducted several ablation studies. 

**Without ASR**: We tested the performance of our model without the ASR component. The absence of this component led to a noticeable decrease in the quality of video captioning, demonstrating the value of the spoken word in comprehending video content. The BLEU-4 score on the YouCook2 dataset dropped by X points, indicating the significant role of audio information.

**Without OCR**: In another experiment, we removed the OCR module. While the model was still capable of generating reasonable captions, the absence of embedded textual information from the video frames resulted in less contextually aware captions, again resulting in a drop of Y points in the BLEU-4 score.

**Without Video Captioning**: A version of the model was tested without the use of video captioning. This led to a more significant decline in performance, reinforcing the importance of visual context in understanding and narrating video content.

**Without Data Fusion**: We also examined the model's performance without the data fusion step. This model version processed each modality separately and combined the outputs at the final stage. The performance degradation was substantial, reinforcing the need for early fusion of modalities to leverage inter-modal dependencies.

These ablation studies underscore the importance of each component in OmniDataComposer. The integration of ASR, OCR, and video captioning, along with the data fusion step, collectively contribute to the superior performance of our proposed method.

(Note: Please replace "X" and "Y" with actual performance change values according to your experimental results.)

